A Study of BERT for Non-Factoid Question-Answering under Passage Length Constraints

We study the use of BERT for non-factoid question-answering, focusing on the passage re-ranking task under varying passage lengths. To this end, we explore the fine-tuning of BERT in different learning-to-rank setups, comprising both point-wise and pair-wise methods, resulting in substantial improvements over the state-of-the-art. We then analyze the effectiveness of BERT for different passage lengths and suggest how to cope with large passages.

==> figs/all_table.tex <==
\begin{table}[h]
	\center
    \small
		\setlength\tabcolsep{1.8pt}
		\caption{Comparison between methods}
		\begin{tabular}{l|c|c||c|c||c|c||c|c|}
			\cline{2-7} 
			\multirow{2}{*}{} & 
				\multicolumn{2}{c||}{\textbf{nfL6}} & 																					\multicolumn{2}{c||}{\textbf{webAP}} & 
				\multicolumn{2}{c||}{\textbf{wikiPsgQA}} \\ 
			\cline{2-7}
 					& P@1 & MRR & P@1 & MRR & MAP & MRR \\ \hline
					\multicolumn{1}{|l|}{BM25} & .131 & .266 & .300 & .412  & .537 & .626 \\ \hline
					\multicolumn{1}{|l|}{DL Baseline} & .352 & .543 & .353 & .515 & .561 &  .679\\ \hline
					\multicolumn{1}{|l|}{BERT CE loss} & .779  & .860 & .475 & .614 &  .71 & .78 \\ \hline
					\multicolumn{1}{|l|}{BERT point-wise} &  .772 & .862  & .55 & .687 & .736 & .81  \\ \hline
					\multicolumn{1}{|l|}{BERTlets} & .776 & .857 & .525 & .683 & .736 & .81 \\ \hline
				\hline
		\end{tabular}
    \label{tab:all}
\end{table}


==> figs/passage_size_table.tex <==
\begin{table}[h]
	\center
    \small
		\setlength\tabcolsep{1.8pt}
		\caption{Effect of passage size (seq-len)}
		\begin{tabular}{l|c|c||c|c||c|c||c|c|}
			\cline{2-7} 
			\multirow{2}{*}{} & 
				\multicolumn{2}{c||}{\textbf{nfL6}} & 																	\multicolumn{2}{c||}{\textbf{webAP}} & 
				\multicolumn{2}{c||}{\textbf{wikiPsgQA}} \\ 
			\cline{2-7}
 					& P@1 & MRR & P@1 & MRR & MAP & MRR \\ \hline
					\multicolumn{1}{|l|}{BERTlets (64)} & .735 &  .828 & .463 & .626  & .500 & .596 \\ \hline
					\multicolumn{1}{|l|}{BERTlets (128)} & .779 & .859 & .538 & .700 & .67 & .755 \\ \hline
					\multicolumn{1}{|l|}{BERTlets (256)} & .776 & .857  & .525 & .683 & .736 & .81 \\ \hline
					\multicolumn{1}{|l|}{BERTlets (384)} &  &   & .525 & .664 & .714 & .783 \\ \hline
				\hline
		\end{tabular}
    \label{tab:block_size}
\end{table}



==> runtime-table.tex <==

\begin{table}[tbh]
	\begin{center}
    \small
		\begin{tabular}{|l|c|c|}
		    \hline
		        & nfL6 (134K) &  WebAP (64K)\\
			\hline
			 64 & 4:49 & 2:13 \\
			\hline
			 128 & 10:24 & 4:39 \\
			\hline
			 256 & 21:32 & 8:26 \\
			\hline
			 384 & 35:50 & 16:40 \\
			\hline
		\end{tabular}
		\caption{Runtime as a function of passage-length}
         \label{tab:runtime}
       \end{center}
\end{table}

